CARE-MI: Chinese Benchmark for Misinformation Evaluation in Maternity and Infant Care

The recent advances in natural language processing (NLP), have led to a new trend of applying large language models (LLMs) to real-world scenarios. While the latest LLMs are astonishingly fluent when interacting with humans, they suffer from the misinformation problem by unintentionally generating factually false statements. This can lead to harmful consequences, especially when produced within sensitive contexts, such as healthcare. Yet few previous works have focused on evaluating misinformation in the long-form (LF) generation of LLMs, especially for knowledge-intensive topics. Moreover, although LLMs have been shown to perform well in different languages, misinformation evaluation has been mostly conducted in English. To this end, we present a benchmark, CARE-MI, for evaluating LLM misinformation in: 1) a sensitive topic, specifically the maternity and infant care domain; and 2) a language other than English, namely Chinese. Most importantly, we provide an innovative paradigm for building LF generation evaluation benchmarks that can be transferred to other knowledge-intensive domains and low-resourced languages. Our proposed benchmark fills the gap between the extensive usage of LLMs and the lack of datasets for assessing the misinformation generated by these models. It contains 1,612 expert-checked questions, accompanied with human-selected references. Using our benchmark, we conduct extensive experiments and found that current Chinese LLMs are far from perfect in the topic of maternity and infant care. In an effort to minimize the reliance on human resources for performance evaluation, we offer off-the-shelf judgment models for automatically assessing the LF output of LLMs given benchmark questions. Moreover, we compare potential solutions for LF generation evaluation and provide insights for building better automated metrics.

==> 007-Datasheet.tex <==
\newpage
\section*{Datasheet} 

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!60!black]
    MOTIVATION
\end{tcolorbox}

\textcolor{blue!60!black}{\textbf{For what purpose was the dataset created?}}

We propose CARE-MI to evaluate the misinformation in the long-form (LF) generation of Chinese LLMs in the maternity and infant care domain. As far as we know, this is the first Chinese benchmark that aims to quantify the misinformation in LF generation scenarios. It is also the only dataset with clear expert annotations on the maternity and infant care domain, and the construction pipeline can be easily transferred to other domains and languages. Our proposed benchmark fills the gap between the extensive usage of LLMs and the lack of datasets for assessing the misinformation generated by LLMs.


\textcolor{blue!60!black}{\textbf{Who created the dataset (e.g., which team, research group) and on behalf of which entity (e.g., company, institution, organization)?}}

The dataset was created by Tong Xiang (Meetyou), Liangzhi Li (Meetyou), 
Wangyue Li (Southwest University of Finance and Economics), Mingbai Bai (Meetyou), Lu Wei (Southwest University of Finance and Economics), Bowen Wang (Osaka University) and Noa Garcia (Osaka University).


\textcolor{blue!60!black}{\textbf{What support was needed to make this dataset?}}

N.A.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!60!black]
    COMPOSITION
\end{tcolorbox}

\textcolor{blue!60!black}{\textbf{What do the instances that comprise the dataset represent (e.g., documents, photos, people, countries)?}}

The instances in this dataset are quadruples; each quadruple contains a question, a default correct answer, a default wrong answer, and several evidence paragraphs. We construct the default correct answer on top existing datasets: BIOS, CPUBMED, MEDQA and MLEC-QA. Questions and default wrong answer are then derived from the default correct answer. The questions include two types, True/False (TF) questions and Open-Ended (OE) questions. Eventually, we retrieve paragraphs from both textbook and Chinese Wikipedia dump which serve as the evidence.

\textcolor{blue!60!black}{\textbf {How many instances are there in total (of each type, if appropriate)?}}

We obtain $79$ instances from BIOS, $497$ instances from CPubMed, $1,634$ instances from MEDQA and $1,349$ instances from MLEC-QA.

\textcolor{blue!60!black}{\textbf{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?}}

The dataset is a selected subset of the originally generated instances. To ensure that the collected data is relevant to the domain of maternity and infant care and having a high quality, we first filter the samples by topic and then apply expert to exclude undesired instances. There are $1,612$ instances kept eventually.
The number of instances in the CARE-MI dataset are as follows:

\begin{table}[h]
\footnotesize
\label{tab-datasheet}
\begin{tabular}{l|rrr}
\toprule
 \textbf{Source}& \textbf{Size}  & \textbf{TF}  & \textbf{OE} \\
\midrule
MLEC-QA  & 567  & 286 &  281  \\
BIOS     & 22  & 22 & -  \\
CPubMed-KG & 150 & 150  &  -  \\
MEDQA   & 873   & 421  &  452  \\
\midrule
All     &  1612  & 879 &  733 \\
\bottomrule
\end{tabular}
\end{table}

\textcolor{blue!60!black}{\textbf{What data does each instance consist of?}}

Each instance in this dataset is a quadruple, consisting of a question, a default correct answer, a default wrong answer, and several supporting paragraphs.

\textcolor{blue!60!black}{\textbf{Is there a label or target associated with each instance?}}

We do not have instance-level label; however, as we are having default correct answer and default wrong answer to the question, we naturally have positive label and negative label for them correspondingly.

\textcolor{blue!60!black}{\textbf{Is any information missing from individual instances?}}

No.

\textcolor{blue!60!black}{\textbf{Are there recommended data splits (e.g., training, development/validation, testing)?}}

No. For our misinformation evaluation, we utilize all samples from the benchmark.

\textcolor{blue!60!black}{\textbf{Are there any errors, sources of noise, or redundancies in the dataset?}}

There are overlaps between the MEDQA and MLEC-QA datasets as they are collected from the same source. We have applied a deduplication process to exclude redundant samples.

\textcolor{blue!60!black}{\textbf{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g., websites, tweets, other datasets)? }}

The dataset is entirely self-contained.

\textcolor{blue!60!black}{\textbf{Does the dataset contain data that might be considered confidential (e.g., data that is protected by legal privilege or by doctor-patient confidentiality, data that includes the content of individuals' non-public communications)?}}

No.

\textcolor{blue!60!black}{\textbf{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?}}

No.

\textcolor{blue!60!black}{\textbf{Does the dataset identify any subpopulations (e.g., by age, gender)?}}

No.

\textcolor{blue!60!black}{\textbf{Is it possible to identify individuals (i.e., one or more natural persons), either directly or indirectly (i.e., in combination with other data) from the dataset? }}

It is impossible to identify individuals from the dataset information.

\textcolor{blue!60!black}{\textbf{Does the dataset contain data that might be considered sensitive in any way (e.g., data that reveals race or ethnic origins, sexual orientations, religious beliefs, political opinions or union memberships, or locations; financial or health data; biometric or genetic data; forms of government identification, such as social security numbers; criminal history)?}}

The dataset does not contain any sensitive information, as all dataset were collected from publicly available sources.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!60!black]
    COLLECTION
\end{tcolorbox}

\textcolor{blue!60!black}{\textbf{How was the data associated with each instance acquired?}}


All data was collected from valid publicly available sources; the samples originally come from either existing knowledge graphs or multiple-choice datasets. To ensure data quality, we additionally hire expert-annotators to filter all the samples we have.

\textcolor{blue!60!black}{\textbf{What mechanisms or procedures were used to collect the data (e.g., hardware apparatuses or sensors, manual human curation, software programs, software APIs)?}}

The data collection procedure can be found in each of the original sources, which we have mentioned in the paper.


\textcolor{blue!60!black}{\textbf{If the dataset is a sample from a larger set, what was the sampling strategy (e.g., deterministic, probabilistic with specific sampling probabilities)?}}

We sample the dataset according to topics, using a pre-defined word-list. To ensure domain relevancy, we manually check each word and only keep those that are highly related to the domain. 

\textcolor{blue!60!black}{\textbf{Who was involved in the data collection process (e.g., students, crowdworkers, contractors) and how were they compensated (e.g., how much were crowdworkers paid)?}}

 All data collection and curation was performed by the paper authors and three medical experts.


\textcolor{blue!60!black}{\textbf{Over what timeframe was the data collected?}}

The dataset was constructed between March 2023 and June 2023. The sources of dataset might have been captured before this timeframe.

\textcolor{blue!60!black}{\textbf{Did you collect the data from the individuals in question directly, or obtain it via third parties or other sources (e.g., websites)?}}

We collect data from two knowledge graph datasets (
 \hyperlink{https://bios.idea.edu.cn/}{BIOS}, \hyperlink{https://cpubmed.openi.org.cn/graph/wiki}{CPubMed}) and two multiple-choice question datasets (\hyperlink{https://github.com/Judenpech/MLEC-QA}{MLEC-QA} and \hyperlink{https://github.com/jind11/MedQA}{MEDQA}) as our data sources. 

\textcolor{blue!60!black}{\textbf{Were the individuals in question notified about the data collection?}}

N.A.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!60!black]
    PREPROCESSING / CLEANING / LABELING
\end{tcolorbox}

\textcolor{blue!60!black}{\textbf{Was the "raw" data saved in addition to the preprocessed/cleaned/labeled data (e.g., to support unanticipated future uses)?}}

Yes, the original data is saved.

\textcolor{blue!60!black}{\textbf{Is the software used to preprocess/clean/label the instances available?}}

Yes, all the codes and software utilized in this project are either open-sourced or commercially available.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!60!black]
    USES
\end{tcolorbox}

\textcolor{blue!60!black}{\textbf{Has the dataset been used for any tasks already?}}

No.

\textcolor{blue!60!black}{\textbf{Is there a repository that links to any or all papers or systems that use the dataset?}}

No for now.

\textcolor{blue!60!black}{\textbf{What (other) tasks could the dataset be used for?}}

The dataset can also be used for fine-tuning conversational capabilities for LLMs.

\textcolor{blue!60!black}{\textbf{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?}} 

Please see the limitation section in the appendix.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!60!black]
    DISTRIBUTION
\end{tcolorbox}

\textcolor{blue!60!black}{\textbf{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?}}

Yes, The dataset will be publicly available on the internet.

\textcolor{blue!60!black}{\textbf{How will the dataset will be distributed (e.g., tarball on website, API, GitHub)?}}

The data will be made public after the review is completed and is currently available in the form of google drive.

\textcolor{blue!60!black}{\textbf{When will the dataset be distributed?}}

The dataset will be publicly available once the reviewing process is finished.

\textcolor{blue!60!black}{\textbf{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?}}

The dataset will be distributed under an Apache License.

\textcolor{blue!60!black}{\textbf{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?}}

No.

\textcolor{blue!60!black}{\textbf{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?}}

No.

\begin{tcolorbox}[colback=blue!5!white,colframe=blue!60!black]
   MAINTENANCE
\end{tcolorbox}

\textcolor{blue!60!black}{\textbf{Who will be supporting/hosting/maintaining the dataset?}}

The dataset is hosted at the Meetyou in Xiamen China. Long-term administrator access is guaranteed for Meetyou.


\textcolor{blue!60!black}{\textbf{How can the owner/curator/manager of the dataset be contacted (e.g., email address)?}}

If any Questions and comments about the datasets, Tong Xiang and Wangyue Li can be contacted at 	xiangtong@xiaoyouzi.com and liwangyue@xiaoyouzi.com, respectively.

\textcolor{blue!60!black}{\textbf{Is there an erratum?}}

No.

\textcolor{blue!60!black}{\textbf{Will the dataset be updated (e.g., to correct labeling errors, add new instances, delete instances)?}} 

Yes the dataset and codes will be updated on a yearly basis.


\textcolor{blue!60!black}{\textbf{Will older versions of the dataset continue to be supported/hosted/maintained?}}

We do not maintain old versions of the dataset, if we update the version of the dataset, we will put the specific details of the dataset update on the relevant GitHub.

\textcolor{blue!60!black}{\textbf{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?}} 

If others want to extend/augment/build on/contribute to the dataset, please contact the authors about incorporating fixes/extensions.

==> 008-Checklist.tex <==
\section*{Checklist}
The Checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Please read the checklist guidelines carefully for information on how to answer these questions. For each question, change the default \textbf{\textcolor{red}{[TODO]}} to \textbf{\textcolor{blue}{[Yes]}}, \textbf{\textcolor{orange}{[No]}}, or \textbf{\textcolor{gray}{[N/A]}}. When answering a question, it is important to provide support for your answer. One way to do this is by referencing the section(s) of the paper that support your answer. Additionally, you can include a brief justification of your answer, which can help the reader understand your thought process and reasoning. By providing additional details and explanations, you can ensure that your answer is clear, thorough, and well-supported. This will help to strengthen your argument and make your paper more convincing overall.

Please refrain from modifying the questions and only use the provided macros to answer them. Note that the Checklist section does not count towards the page limit. When submitting your paper, delete this instruction block and keep only the Checklist section heading along with the questions and answers below.

\begin{itemize}
    \item[1] For all authors...
     \begin{itemize}
         \item [a] Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \textbf{\textcolor{blue}{[Yes]}}
         \item [b] Have you read the ethics review guidelines and ensured that your paper conforms to them? \textbf{\textcolor{blue}{[Yes]}}
         \item[c] Did you discuss any potential negative societal impacts of your work?
         \textbf{\textcolor{blue}{[Yes]}} Please see Appendix.
         \item[d] Did you describe the limitations of your work?   \textbf{\textcolor{blue}{[Yes]}} Please see Appendix.
     \end{itemize}
     \item[2] If you are including theoretical results...
     \begin{itemize}
         \item [a] Did you state the full set of assumptions of all theoretical results? \textbf{\textcolor{gray}{[N/A]}}
         \item [b] Did you include complete proofs of all theoretical results? \textbf{\textcolor{gray}{[N/A]}}
     \end{itemize}
      \item[3] If you ran experiments...
       \begin{itemize}
         \item [a] Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
 \textbf{\textcolor{blue}{[Yes]}} All the benchmarks and codes are available at \url{https://github.com/Meetyou-AI-Lab/CARE-MI}, and the data will be made public after the review is completed and is currently available in the form of google drive.
         \item [b] Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
 \textbf{\textcolor{blue}{[Yes]}} Those details were listed in Section 3 and Section 4.3.
         \item[c] Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
         \textbf{\textcolor{orange}{[No]}} We evaluated several LLMs on our proposed benchmark with respect to misinformation in LF generation. All experiments were conducted in the form of a single-round conversation, we only set the temperature parameter here. 
        \item[d] Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
         \textbf{\textcolor{blue}{[Yes]}} We share our experimental settings at Appendix.
     \end{itemize}
     \item[4] If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
     \begin{itemize}
         \item [a] If your work uses existing assets, did you cite the creators? \textbf{\textcolor{blue}{[Yes]}} All the sources were properly cited in this paper.
         \item [b] Did you mention the license of the assets? \textbf{\textcolor{orange}{[No]}} The code we used are all open available, we do not claim any copyright from the code.
         \item[c] Did you include any new assets either in the supplemental material or as a URL?
         \textbf{\textcolor{blue}{[Yes]}}
         \item[d] Did you discuss whether and how consent was obtained from people whose data you're using/curating? 
         \textbf{\textcolor{blue}{[Yes]}}
         As this work was conducted on publicly available data, participant consent is waived for this study.
         \item[e] Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content? 
         \textbf{\textcolor{blue}{[Yes]}} This work is completely devoid of any personally identifiable information or offensive content.
     \end{itemize}
     \item[5] If you used crowdsourcing or conducted research with human subjects...
      \begin{itemize}
         \item [a] Did you include the full text of instructions given to participants and screenshots, if applicable? \textbf{\textcolor{gray}{[N/A]}} This work was conducted using publicly available data and does not involve any participants.
         \item [b] Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable? \textbf{\textcolor{gray}{[N/A]}}
         Our dataset is based on National
103 Medical Licensing Examination in China (NMLEC), National Library of Medicine, Chinese Wikipedia and medical boooks, so they don't have potential participant risks.
         \item[c] Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
         \textbf{\textcolor{orange}{[No]}} This dataset was voluntarily annotated by the authors and three medical experts.
     \end{itemize}
\end{itemize}
